A new class of one-step A-stable and L-stable schemes of high-order accuracy for parabolic type equations

Recently, a new class of BDF schemes proposed in [F. Huang and J. Shen, SIAM J Numer. Anal., 62.4, 1609--1637] for the parabolic type equations are studied in this paper. The basic idea is based on the Taylor expansions at time $t^{n+\beta}$ with $\beta>1$ being a tunable parameter. These new BDF schemes allow larger time steps at higher order r for stiff problems than that which allowed with a usual higher-order scheme. However, multi-step methods like BDF exhibit inherent disadvantages relative to one-step methods in practical implementations. In this paper, inspired by their excellent work, we construct a new class of high-order one-step schemes for linear parabolic-type equations. These new schemes, with several suitable $\beta_i$, can achieve A-stable, or even L-stable. Specially, the new scheme with special parameters $\beta_i$ can be regarded as the classical one-step Runge-Kutta scheme with a stabilized term. Besides, we provide two different techniques to construct the one-step high-order schemes: the first one is by choosing different parameters $\beta_i$, and the second one is by increasing the number of intermediate layers. Both methods have been proven to be highly effective and even exhibit superconvergence property. Finally, we also conducted several numerical experiments to support our conclusions.

==> q.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{baer1998heat}
\citation{gassner2008discontinuous}
\citation{GASSNER20071049}
\citation{dumbser2009high}
\citation{aslam1996level}
\citation{markstein2014nonsteady}
\citation{rubinshteuin1971stefan}
\citation{balsara2008simulating}
\citation{osher2004level}
\citation{sethian1999level}
\citation{hochbruck2005exponential}
\citation{ju2021maximum}
\citation{martin2016extrapolated}
\citation{meyer2014stabilized}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}\protected@file@percent }
\citation{huang2024new}
\newlabel{eq1}{{1.1}{2}{Introduction}{equation.2}{}}
\newlabel{eq1@cref}{{[equation][1][1]1.1}{[1][2][]2}}
\@writefile{toc}{\contentsline {section}{\numberline {2}A brief review of GBDF scheme and Runge-Kutta scheme}{3}{section.3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}The GBDF scheme}{3}{subsection.4}\protected@file@percent }
\newlabel{2.2}{{2.2}{3}{The GBDF scheme}{equation.6}{}}
\newlabel{2.2@cref}{{[equation][2][2]2.2}{[1][3][]3}}
\newlabel{2.3}{{2.4}{3}{The GBDF scheme}{equation.8}{}}
\newlabel{2.3@cref}{{[equation][4][2]2.4}{[1][3][]3}}
\citation{akrivis2016backward}
\citation{akrivis2015fully}
\citation{li2020long}
\newlabel{2.4}{{2.5}{4}{The GBDF scheme}{equation.10}{}}
\newlabel{2.4@cref}{{[equation][5][2]2.5}{[1][4][]4}}
\@writefile{thm}{\contentsline {remark}{{Remark}{2.1}{}}{4}{theorem.14}\protected@file@percent }
\citation{hairer1993sp}
\citation{wanner1996solving}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Runge-Kutta scheme}{5}{subsection.15}\protected@file@percent }
\newlabel{RK_scheme}{{2.6}{5}{Runge-Kutta scheme}{equation.16}{}}
\newlabel{RK_scheme@cref}{{[equation][6][2]2.6}{[1][4][]5}}
\@writefile{toc}{\contentsline {section}{\numberline {3}The new one-step schemes}{5}{section.20}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}The first high-order one-step scheme}{5}{subsection.21}\protected@file@percent }
\newlabel{taylor}{{3.1}{5}{The first high-order one-step scheme}{equation.22}{}}
\newlabel{taylor@cref}{{[equation][1][3]3.1}{[1][5][]5}}
\newlabel{eq2}{{3.3}{6}{The first high-order one-step scheme}{equation.24}{}}
\newlabel{eq2@cref}{{[equation][3][3]3.3}{[1][6][]6}}
\newlabel{A value}{{3.5}{6}{The first high-order one-step scheme}{equation.26}{}}
\newlabel{A value@cref}{{[equation][5][3]3.5}{[1][6][]6}}
\newlabel{eq3}{{3.6}{6}{The first high-order one-step scheme}{equation.27}{}}
\newlabel{eq3@cref}{{[equation][6][3]3.6}{[1][6][]6}}
\newlabel{A value}{{3.8}{6}{The first high-order one-step scheme}{equation.29}{}}
\newlabel{A value@cref}{{[equation][8][3]3.8}{[1][6][]6}}
\newlabel{equal-system}{{3.9}{7}{The first high-order one-step scheme}{equation.30}{}}
\newlabel{equal-system@cref}{{[equation][9][3]3.9}{[1][6][]7}}
\newlabel{one-step-eq1}{{3.10}{7}{The first high-order one-step scheme}{equation.31}{}}
\newlabel{one-step-eq1@cref}{{[equation][10][3]3.10}{[1][7][]7}}
\newlabel{one-step-eq2}{{3.12}{7}{The first high-order one-step scheme}{equation.33}{}}
\newlabel{one-step-eq2@cref}{{[equation][12][3]3.12}{[1][7][]7}}
\newlabel{one-step-eq3}{{3.13}{7}{The first high-order one-step scheme}{equation.34}{}}
\newlabel{one-step-eq3@cref}{{[equation][13][3]3.13}{[1][7][]7}}
\newlabel{one-step-eq4}{{3.14}{7}{The first high-order one-step scheme}{equation.35}{}}
\newlabel{one-step-eq4@cref}{{[equation][14][3]3.14}{[1][7][]7}}
\newlabel{eq4}{{3.15}{7}{The first high-order one-step scheme}{equation.36}{}}
\newlabel{eq4@cref}{{[equation][15][3]3.15}{[1][7][]7}}
\newlabel{eq5}{{3.17}{8}{The first high-order one-step scheme}{equation.38}{}}
\newlabel{eq5@cref}{{[equation][17][3]3.17}{[1][7][]8}}
\newlabel{expandeq}{{3.21}{8}{The first high-order one-step scheme}{equation.42}{}}
\newlabel{expandeq@cref}{{[equation][21][3]3.21}{[1][8][]8}}
\@writefile{thm}{\contentsline {theorem}{{Theorem}{3.1}{}}{9}{theorem.45}\protected@file@percent }
\@writefile{thm}{\contentsline {proof}{{Proof}{1}{}}{9}{proof.48}\protected@file@percent }
\newlabel{one-step-eq5}{{3.29}{9}{The first high-order one-step scheme}{equation.52}{}}
\newlabel{one-step-eq5@cref}{{[equation][29][3]3.29}{[1][9][]9}}
\newlabel{one-step-eq6}{{3.30}{9}{The first high-order one-step scheme}{equation.53}{}}
\newlabel{one-step-eq6@cref}{{[equation][30][3]3.30}{[1][9][]9}}
\newlabel{one-step-eq7}{{3.31}{10}{The first high-order one-step scheme}{equation.54}{}}
\newlabel{one-step-eq7@cref}{{[equation][31][3]3.31}{[1][9][]10}}
\global\def\markiproofvii{\proofbox }
\@writefile{thm}{\contentsline {theorem}{{Theorem}{3.2}{}}{10}{theorem.56}\protected@file@percent }
\newlabel{eq-system}{{3.33}{10}{The first high-order one-step scheme}{equation.57}{}}
\newlabel{eq-system@cref}{{[equation][33][3]3.33}{[1][10][]10}}
\@writefile{thm}{\contentsline {proof}{{Proof}{2}{}}{10}{proof.58}\protected@file@percent }
\newlabel{mRK_2}{{3.35}{10}{The first high-order one-step scheme}{equation.60}{}}
\newlabel{mRK_2@cref}{{[equation][35][3]3.35}{[1][10][]10}}
\global\def\markiiproofvii{\proofbox }
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}The second high-order one-step scheme}{11}{subsection.66}\protected@file@percent }
\newlabel{taylor3}{{3.41}{11}{The second high-order one-step scheme}{equation.67}{}}
\newlabel{taylor3@cref}{{[equation][41][3]3.41}{[1][11][]11}}
\newlabel{eqthird}{{3.42}{12}{The second high-order one-step scheme}{equation.68}{}}
\newlabel{eqthird@cref}{{[equation][42][3]3.42}{[1][11][]12}}
\newlabel{eq8}{{3.43}{12}{The second high-order one-step scheme}{equation.69}{}}
\newlabel{eq8@cref}{{[equation][43][3]3.43}{[1][12][]12}}
\newlabel{eqthird2}{{3.45}{12}{The second high-order one-step scheme}{equation.71}{}}
\newlabel{eqthird2@cref}{{[equation][45][3]3.45}{[1][12][]12}}
\newlabel{eq9}{{3.46}{12}{The second high-order one-step scheme}{equation.72}{}}
\newlabel{eq9@cref}{{[equation][46][3]3.46}{[1][12][]12}}
\newlabel{eq10}{{3.48}{12}{The second high-order one-step scheme}{equation.74}{}}
\newlabel{eq10@cref}{{[equation][48][3]3.48}{[1][12][]12}}
\newlabel{eq11}{{3.49}{13}{The second high-order one-step scheme}{equation.75}{}}
\newlabel{eq11@cref}{{[equation][49][3]3.49}{[1][12][]13}}
\@writefile{thm}{\contentsline {remark}{{Remark}{3.3}{}}{14}{theorem.81}\protected@file@percent }
\@writefile{thm}{\contentsline {remark}{{Remark}{3.4}{}}{14}{theorem.82}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {4}Stability analysis of (\ref {eq5})}{14}{section.83}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Stability of second-order scheme}{14}{subsection.84}\protected@file@percent }
\newlabel{eq7}{{4.1}{14}{Stability of second-order scheme}{equation.85}{}}
\newlabel{eq7@cref}{{[equation][1][4]4.1}{[1][14][]14}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=-\frac  13$.}}{14}{figure.87}\protected@file@percent }
\newlabel{stable_ex1}{{1}{14}{The green parts show the region of absolute stability of the new schemes with $\beta _1=-\frac 13$}{figure.87}{}}
\newlabel{stable_ex1@cref}{{[figure][1][]1}{[1][14][]14}}
\@writefile{thm}{\contentsline {theorem}{{Theorem}{4.1}{}}{14}{theorem.95}\protected@file@percent }
\newlabel{teq1}{{4.4}{14}{Stability of second-order scheme}{equation.97}{}}
\newlabel{teq1@cref}{{[equation][4][4]4.4}{[1][14][]14}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=0$.}}{15}{figure.89}\protected@file@percent }
\newlabel{stable_ex2}{{2}{15}{The green parts show the region of absolute stability of the new schemes with $\beta _1=0$}{figure.89}{}}
\newlabel{stable_ex2@cref}{{[figure][2][]2}{[1][14][]15}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac  13$.}}{15}{figure.91}\protected@file@percent }
\newlabel{stable_ex3}{{3}{15}{The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac 13$}{figure.91}{}}
\newlabel{stable_ex3@cref}{{[figure][3][]3}{[1][14][]15}}
\@writefile{thm}{\contentsline {proof}{{Proof}{3}{}}{15}{proof.98}\protected@file@percent }
\newlabel{teq2}{{4.5}{15}{Stability of second-order scheme}{equation.99}{}}
\newlabel{teq2@cref}{{[equation][5][4]4.5}{[1][14][]15}}
\@writefile{thm}{\contentsline {theorem}{{Theorem}{4.2}{}}{15}{theorem.103}\protected@file@percent }
\newlabel{teq3}{{4.9}{15}{Stability of second-order scheme}{equation.104}{}}
\newlabel{teq3@cref}{{[equation][9][4]4.9}{[1][15][]15}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac  12-\frac  {\sqrt  3}6$.}}{16}{figure.93}\protected@file@percent }
\newlabel{stable_ex4}{{4}{16}{The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac 12-\frac {\sqrt 3}6$}{figure.93}{}}
\newlabel{stable_ex4@cref}{{[figure][4][]4}{[1][14][]16}}
\newlabel{teq4}{{4.10}{16}{Stability of second-order scheme}{equation.105}{}}
\newlabel{teq4@cref}{{[equation][10][4]4.10}{[1][15][]16}}
\@writefile{thm}{\contentsline {proof}{{Proof}{4}{}}{16}{proof.106}\protected@file@percent }
\newlabel{teq5}{{4.11}{16}{Stability of second-order scheme}{equation.107}{}}
\newlabel{teq5@cref}{{[equation][11][4]4.11}{[1][16][]16}}
\@writefile{thm}{\contentsline {theorem}{{Theorem}{4.3}{}}{16}{theorem.112}\protected@file@percent }
\newlabel{teq6}{{4.16}{16}{Stability of second-order scheme}{equation.113}{}}
\newlabel{teq6@cref}{{[equation][16][4]4.16}{[1][16][]16}}
\newlabel{teq7}{{4.17}{17}{Stability of second-order scheme}{equation.114}{}}
\newlabel{teq7@cref}{{[equation][17][4]4.17}{[1][16][]17}}
\@writefile{thm}{\contentsline {proof}{{Proof}{5}{}}{17}{proof.115}\protected@file@percent }
\global\def\markvproofi{\proofbox }
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Stability regions of third-order scheme}{17}{subsection.117}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=-\frac  14,\tmspace  +\thickmuskip {.2777em}\beta _2=\frac  12$.}}{17}{figure.119}\protected@file@percent }
\newlabel{stable_3order_ex1}{{5}{17}{The green parts show the region of absolute stability of the new schemes with $\beta _1=-\frac 14,\;\beta _2=\frac 12$}{figure.119}{}}
\newlabel{stable_3order_ex1@cref}{{[figure][5][]5}{[1][17][]17}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=0,\tmspace  +\thickmuskip {.2777em}\beta _2=\frac  12$.}}{17}{figure.121}\protected@file@percent }
\newlabel{stable_3order_ex2}{{6}{17}{The green parts show the region of absolute stability of the new schemes with $\beta _1=0,\;\beta _2=\frac 12$}{figure.121}{}}
\newlabel{stable_3order_ex2@cref}{{[figure][6][]6}{[1][17][]17}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac  14,\tmspace  +\thickmuskip {.2777em}\beta _2=\frac  12$.}}{18}{figure.123}\protected@file@percent }
\newlabel{stable_3order_ex3}{{7}{18}{The green parts show the region of absolute stability of the new schemes with $\beta _1=\frac 14,\;\beta _2=\frac 12$}{figure.123}{}}
\newlabel{stable_3order_ex3@cref}{{[figure][7][]7}{[1][17][]18}}
\@writefile{toc}{\contentsline {section}{\numberline {5}Numerical examples}{18}{section.125}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces The exact solution and the numerical solution obtained by the second-order scheme with different $\beta _1$, $\beta _2$ and $\lambda $.}}{18}{figure.127}\protected@file@percent }
\newlabel{ex1}{{8}{18}{The exact solution and the numerical solution obtained by the second-order scheme with different $\beta _1$, $\beta _2$ and $\lambda $}{figure.127}{}}
\newlabel{ex1@cref}{{[figure][8][]8}{[1][18][]18}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces The images of the convergence order for parameter $\beta _1$ under different conditions.}}{19}{figure.130}\protected@file@percent }
\newlabel{ex2_1}{{9}{19}{The images of the convergence order for parameter $\beta _1$ under different conditions}{figure.130}{}}
\newlabel{ex2_1@cref}{{[figure][9][]9}{[1][19][]19}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces The superconvergence image of the second-order scheme.}}{19}{figure.132}\protected@file@percent }
\newlabel{ex2_2}{{10}{19}{The superconvergence image of the second-order scheme}{figure.132}{}}
\newlabel{ex2_2@cref}{{[figure][10][]10}{[1][19][]19}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces The images of the convergence order of the third-order scheme under different $\beta $.}}{19}{figure.134}\protected@file@percent }
\newlabel{ex2_3}{{11}{19}{The images of the convergence order of the third-order scheme under different $\beta $}{figure.134}{}}
\newlabel{ex2_3@cref}{{[figure][11][]11}{[1][19][]19}}
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces The reference solution of Example 3.}}{20}{figure.137}\protected@file@percent }
\newlabel{ex3_1}{{12}{20}{The reference solution of Example 3}{figure.137}{}}
\newlabel{ex3_1@cref}{{[figure][12][]12}{[1][20][]20}}
\@writefile{toc}{\contentsline {section}{\numberline {6}Concluding remarks}{20}{section.146}\protected@file@percent }
\citation{*}
\bibstyle{plain}
\bibdata{baer1998heat,S0021999106005651,gassner2008discontinuous,dumbser2009high,aslam1996level,markstein2014nonsteady,rubinshteuin1971stefan,balsara2008simulating,osher2004level,sethian1999level,ju2021maximum,martin2016extrapolated,meyer2014stabilized,hochbruck2005exponential,huang2024new,akrivis2016backward,akrivis2015fully,li2020long,hairer1993sp,wanner1996solving}
\bibcite{akrivis2016backward}{1}
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces The numerical solution of Example 3.}}{21}{figure.139}\protected@file@percent }
\newlabel{ex3_2}{{13}{21}{The numerical solution of Example 3}{figure.139}{}}
\newlabel{ex3_2@cref}{{[figure][13][]13}{[1][20][]21}}
\@writefile{lof}{\contentsline {figure}{\numberline {14}{\ignorespaces The reference solution of Example 4.}}{21}{figure.142}\protected@file@percent }
\newlabel{ex4_1}{{14}{21}{The reference solution of Example 4}{figure.142}{}}
\newlabel{ex4_1@cref}{{[figure][14][]14}{[1][20][]21}}
\@writefile{toc}{\contentsline {section}{References}{21}{section.146}\protected@file@percent }
\bibcite{akrivis2015fully}{2}
\bibcite{aslam1996level}{3}
\bibcite{baer1998heat}{4}
\bibcite{balsara2008simulating}{5}
\bibcite{dumbser2009high}{6}
\bibcite{gassner2008discontinuous}{7}
\bibcite{GASSNER20071049}{8}
\bibcite{hairer1993sp}{9}
\bibcite{hochbruck2005exponential}{10}
\bibcite{huang2024new}{11}
\bibcite{ju2021maximum}{12}
\bibcite{li2020long}{13}
\bibcite{markstein2014nonsteady}{14}
\bibcite{martin2016extrapolated}{15}
\bibcite{meyer2014stabilized}{16}
\@writefile{lof}{\contentsline {figure}{\numberline {15}{\ignorespaces The numerical solution of Example 4.}}{22}{figure.144}\protected@file@percent }
\newlabel{ex4_2}{{15}{22}{The numerical solution of Example 4}{figure.144}{}}
\newlabel{ex4_2@cref}{{[figure][15][]15}{[1][20][]22}}
\bibcite{osher2004level}{17}
\bibcite{rubinshteuin1971stefan}{18}
\bibcite{sethian1999level}{19}
\bibcite{wanner1996solving}{20}
\gdef \@abspage@last{23}

